Human-Robot Kinaesthetic Interaction Based on Free Energy Principle

The current study investigated possible human-robot kinaesthetic interaction using a variational recurrent neural network model, called PV-RNN, which is based on the free energy principle. Our prior robotic studies using PV-RNN showed that the nature of interactions between top-down expectation and bottom-up inference is strongly affected by a parameter, called the meta-prior, which regulates the complexity term in free energy.The study also compares the counter force generated when trained transitions are induced by a human experimenter and when untrained transitions are induced. Our experimental results indicated that (1) the human experimenter needs more/less force to induce trained transitions when $w$ is set with larger/smaller values, (2) the human experimenter needs more force to act on the robot when he attempts to induce untrained as opposed to trained movement pattern transitions. Our analysis of time development of essential variables and values in PV-RNN during bodily interaction clarified the mechanism by which gaps in actional intentions between the human experimenter and the robot can be manifested as reaction forces between them.

==> 6_bibliography.tex <==
\begin{thebibliography}{1}
\bibliographystyle{IEEEtran}

\bibitem{psychology}
L. S. Vygotsky, {\it{Mind in society: The development of higher psychological processes}}. Harvard university press, 1980.



\bibitem{DL_to_ToM}
Aru, Jaan et al. (2022). Mind the gap: Challenges of deep learning approaches to Theory of Mind. {\it{ArXiv}} abs/2203.16540.

\bibitem{FEP_recent_study1}
Friston, K. (2018). Does predictive coding have a future? {\it{Nature neuroscience}}, 21(8), 1019.

\bibitem{FEP_recent_study2}
A. Clark, {\it{Surfing Uncertainty: Prediction, Action, ad the embodied Mind.}} London, U.K.: Oxford Univ. Press, 2015. (2018). Does predictive coding have a future? {/it{Nature neuroscience}}, 21(8), 1019.

\bibitem{PV-RNN}
Ahmadreza Ahmadi, Jun Tani; A Novel Predictive-Coding-Inspired Variational RNN Model for Online Prediction and Recognition. {\it{Neural Comput}} 2019; 31 (11): 2025–2074.

\bibitem{Model_based_on_FEP1}
S. Murata, Y. Yamashita, H. Arie, T. Ogata, S. Sugano, and J. Tani, “Learning to perceive the world as probabilistic or deterministic via interaction with others: A neuro-robotics experiment,” {\it{IEEE Trans. Neural Netw. Learn. Syst.}}, vol. 28, no. 4, pp. 830–848, Apr. 2017.

\bibitem{Model_based_on_FEP2}
P. Lanillos and G. Cheng, “Adaptive Robot Body Learning and Estimation Through Predictive Coding,” {\it{CoRR}}, vol. abs/1805.03104, 2018.

\bibitem{Model_based_on_FEP3}
C. Lang, G. Schillaci, and V. Hafner, “A deep convolutional neural network model for sense of agency and object permanence in robots,” in {\it{Proc. Joint IEEE 8th Int. Conf. Develop. Learn. Epigenetic Robot.}} (ICDL-EpiRob), pp. 257–262, 2018.

\bibitem{Model_based_on_FEP4}
A. Philippsen and Y. Nagai, “Deficits in prediction ability trigger asymmetries in behavior and internal representation,” {\it{Front. Psychiatry}}, vol. 11, p. 1253, 2020.

\bibitem{Model_based_on_FEP5}
Chung, J., Kastner, K., Dinh, L., Goel, K., Courville, A. C., & Bengio, Y. (2015). A recurrent latent variable model for sequential data. In {\it{Advances in neural information processing systems}} (pp. 2980–2988).

\bibitem{Hendry}
Chame, Hendry F., and Jun Tani (2020). Cognitive and motor compliance in intentional human-robot interaction. {\it{2020 IEEE International Conference on Robotics and Automation (ICRA).}}

\bibitem{FreeEnergyPrinciple}
Friston, K (2010). The free-energy principle: a unified brain theory?. {\it{Nat Rev Neurosci}}, vol. 11, p. 127–138.

\bibitem{Idei}
Idei, H., Ohata, W., Yamashita, Y. et al. Emergence of sensory attenuation based upon the free-energy principle. {\it Sci Rep}, 12, 14542 (2022). https://doi.org/10.1038/s41598-022-18207-7

\bibitem{Takazumi}
Takazumi M., Wataru O., et al. Goal-Directed Planning and Goal Understanding by Extended Active Inference: Evaluation through Simulated and Physical Robot Experiments. {\it Entropy}, Vol. 24, Issue 4 (2022).

\end{thebibliography}
